Online Residual Learning from Offline Experts for Pedestrian Tracking

In this paper, we consider the problem of predicting unknown targets from data. We propose Online Residual Learning (ORL), a method that combines online adaptation with offline-trained predictions. At a lower level, we employ multiple offline predictions generated before or at the beginning of the prediction horizon. We augment every offline prediction by learning their respective residual error concerning the true target state online, using the recursive least squares algorithm. At a higher level, we treat the augmented lower-level predictors as experts, adopting the Prediction with Expert Advice framework. We utilize an adaptive softmax weighting scheme to form an aggregate prediction and provide guarantees for ORL in terms of regret. We employ ORL to boost performance in the setting of online pedestrian trajectory prediction. Based on data from the Stanford Drone Dataset, we show that ORL can demonstrate best-of-both-worlds performance.

==> sections/backup.tex <==
\subsection{Residual Error Learning}
% \tasos{I am not sure if this is what we assume. I guess it is rather that the residuals are time-varying. Or we could say that we are motivated by first-order approximations: linearizing around every expert we obtain
% \[
% r_{t+1}-\hat{r}^{\mathrm{off}}_{t+1,i}=\frac{d f(x)}{d x}|_{x=r_{t-p+1:t}}(r_{t-p+1:t}-\hat{r}^{\mathrm{off}}_{t-p+1:t,i})+w_{t,i}
% \]
% where the first component is the Jacobian and the second is the linearization error. This motivates us to consider models for the residuals as....
% }\eb{Do we need to state it like this? I'd put this later as an interpretation, I think here the only idea we have is there's some base model and model mismatch residual we want to learn which is quite standard in many applications. Also maybe $\partial$ instead of derivatives since we don't assume smoothness etc., (I know this is a high-level idea).}
% \tasos{Also not sure if we should present this as a model. We should rather state the RLS component here and then the meta learner. I guess the material of subsection c should be here.}
The offline predictions might be good initial guesses, but they do not adapt to the target's motion; additional online correction might be needed. Define the residual errors between the offline predictions and the true target state as:
\begin{equation}
    e_{t,i} \triangleq r_t - \hat{r}_{t,i}^{\mathrm{off}} 
    \label{eq:res_error}
\end{equation}
where $r_t$ is the (sequentially revealed) target state and $i\in\{1,2,\dots,N\}$ is the expert index. The main idea is to augment every expert $i$ by learning online their respective residual error $e_{t,i}$. Let $\hat{e}_{t+k,i}$ denote the prediction of the $k-$steps ahead residual error at time $t$. Then, at every time step $t$, every expert $i$ outputs the corrected prediction 
\begin{equation}\label{eq:augmented_expert_prediction}
\hat{r}_{t+k,i}\triangleq\hat{e}_{t+k,i}+\hat{r}^\mathrm{off}_{t+k,i},\,i\in\{1,2,\dots,N\}. 
\end{equation}
Then, the loss of each expert is equal to
\[
\ell_t(\hat{r}_{t,i})=\|r_t-(\hat{e}_{t,i}+\hat{r}^{\mathrm{off}}_{t,i}) \|^2 =\|  e_{t,i}-\hat{e}_{t,i}\|^2.
\]
This implies that we can perform online regression on the residuals $e_{t,i}$ instead of performing online regression on the target state $r_t$ directly. 

Online Residual Learning predicts the residual errors by employing the Recursive Least Squares (RLS) algorithm, which aims to find the best possible \emph{linear} predictor. At every time $0\le t\le T$, every expert $i\in\{1,2,\dots,N\}$ minimizes the following cost:
\begin{equation}
\begin{aligned}
 \hat{M}_{t,i}=\arg\min_{M\in\mathcal{S}}   J_t(M) &\triangleq \sum_{\tau=p+k-1}^t \gamma_i^{t-\tau} \norm{e_{\tau,i} - M z_{\tau-k,i}}^2,\\
    z_{\tau-k,i}&=e_{\tau-k-p+1:\tau-k,i}
    \label{eq:cost}
    \end{aligned}
\end{equation}
and predicts
\begin{equation}\label{eq:RLS_prediciton}
\hat{e}_{t+k,i}=\hat{M}_{t+k,i}z_{t,i}.
\end{equation}
\tasos{not fully accurate since the different learners are not explained}
Notice that we introduce forgetting factors $\gamma_i\in(0,1]$ to adapt to changing dynamics and a constraint set $\mathcal{S}$. % where $\ell_t(M_i) = \norm{e_{t,i} - M_ie_{t-k,i}}^2 $ 
A recursive update is given in \cref{alg:RLS}. 

We make the following standard assumptions \cite{yuan2020trading} to guarantee that the RLS algorithm is well-behaved.
\begin{assumption}\label{assum:bounded_residuals}
    The residual errors are bounded, i.e. for some $D_r\geq 0$, $\norm{e_{t,i}} \leq D_r$ , for all $1\leq t\leq T$, $i\in\{1,2,\dots,N\}$.
\end{assumption}
\begin{assumption}
    Let $\mathcal{S} \triangleq \{S\in\mathbb{R}^{n\times np}| \norm{S}\leq D\}$ for some $D\geq 0$. The $k$-step ahead dynamics \ref{eq:k-step-ahead-dynamics} are uniformly bounded: $M_{t+k|t,i} \in S $ for all $0\leq t \leq T$, $i\in\{1,2,\dots,N\}$.
\end{assumption}

We note that the RLS algorithm does not require the underlying process, in our case $e_{t,i}$, to obey linear dynamics. It will achieve a competing performance compared to the best linear predictors, even if the residual errors evolve in a non-linear fashion. Besides, given \cref{assum:bounded_residuals}, there always exist $M_{t,i}$ and $w_{t,i}$ such that the residual errors act as an affine time-varying dynamical system of the form:
\begin{equation*}
    e_{t+k,i} = M_{t,i}e_{t-p+1:t,i} + w_{t,i}
    \label{eq:error_affine}
\end{equation*}

We assume that the offline predictions $\hat{r}_{t,i}^{\mathrm{off}}$ have some dynamics of the form
\begin{equation}
    \hat{r}_{t+1,i}^{\mathrm{off}} = f_{\mathrm{off}}(\hat{r}_{t-p+1:t,i}^{\mathrm{off}}) 
\end{equation}
From \eqref{eq:res_error}, we get that:
\begin{align}
    \begin{split}
        r_{t+1} - \hat{r}^{\mathrm{off}}_{t+1,i} &= f(r_{t-p+1:t}) - f_{\mathrm{off}}(\hat{r}_{t-p+1:t,i}^{\mathrm{off}}) \\
        &= f(r_{t-p+1:t}) - f(\hat{r}_{t-p+1:t,i}^{\mathrm{off}}) \\
        &+ f(\hat{r}_{t-p+1:t,i}^{\mathrm{off}}) - f_{\mathrm{off}}(\hat{r}_{t-p+1:t,i}^{\mathrm{off}}) \\
        &\approx \left.\frac{\partial f(x)}{\partial x}\right|_{x = r_{t-p+1:t}} (r_{t-p+1:t} - \hat{r}_{t-p+1:t,i}^{\mathrm{off}}) \\
        &+ \norm{f-f_{\mathrm{off}}}(\hat{r}_{t-p+1:t,i}^{\mathrm{off}})
        % \frac{d f(x)}{d x}|_{x=r_{t-p+1:t}}(r_{t-p+1:t}-\hat{r}^{\mathrm{off}}_{t-p+1:t,i})+w_{t,i} 
    \end{split}
\end{align}
Therefore, we can say that the residual errors act as an affine time-varying dynamical system of the form:
\begin{equation}
    e_{t+1,i} = M_{t,i}e_{t-p+1:t,i} + w_{t,i}
    \label{eq:error_affine}
\end{equation}
where $e_{t-p+1:t,i} = r_{t-p+1:t} - \hat{r}_{t-p+1:t,i}^{\mathrm{off}}$, $M_{t,i} = \left.\frac{\partial f(x)}{\partial x}\right|_{x = r_{t-p+1:t}}$ is the \emph{Jacobian} of $f$ computed at $r_{t-p+1:t}$ and $w_{t,i} = \norm{f-f_{\mathrm{off}}}(\hat{r}_{t-p+1:t,i}^{\mathrm{off}})$ is the linearization error. These can be written as a Linear Time-Varying (LTV) system if we consider the augmented state $\Tilde{e}_{t,i} = \begin{bmatrix}
    e_{t,i}^{\top} & 1
\end{bmatrix}^{\top}$ and $\Tilde{M}_{t,i} = \begin{bmatrix}
    M_{t,i} & w_{t,i}
\end{bmatrix}$:
\begin{equation}
    \Tilde{e}_{t+1,i} = \Tilde{M}_{t,i}\Tilde{e}_{t-p+1:t,i}
    \label{eq:error_ltv}
\end{equation}

For simplicity reasons, from this point forward, we will drop the $\Tilde{\cdot}$ notation and we will assume the LTV system in the augmented state space. Applying $k$ times the model \eqref{eq:error_ltv} we get the $k$-step ahead model:
\begin{equation}
    e_{t+k,i} = M_{t+k|t,i}e_{t-p+1:t,i}
    \label{eq:k-step-ahead-dynamics}
\end{equation}
where $M_{t+k|t}$ is a nonlinear combination of $M_{t+k}, \dots, M_t$.

% Moreover, we will make some common assumptions \cite{yuan2020trading} that reflect the boundedness of dynamics \ref{eq:error_ltv}:
% \begin{assumption}
%     The residual errors are bounded, i.e. for some $D_r\geq 0$, $\norm{e_{t,i}} \leq D_r$ , for all $1\leq t\leq T$, $i\in\{1,2,\dots,N\}$.
% \end{assumption}
% \begin{assumption}
%     Let $\mathcal{S} \triangleq \{S\in\mathbb{R}^{n\times np}| \norm{S}\leq D\}$ for some $D\geq 0$. The $k$-step ahead dynamics \ref{eq:k-step-ahead-dynamics} are uniformly bounded: $M_{t+k|t,i} \in S $ for all $0\leq t \leq T$, $i\in\{1,2,\dots,N\}$.
% \end{assumption}

% In this work, we assume that the data we wish to predict is generated by \textit{time-varying}, \textit{auto-regressive} dynamics of the form:
% \begin{equation}
%     r_{t+1} = M_t r_{t,p}
%     \label{eq:dynamics}
% \end{equation}
% where 
% \begin{equation}
%     r_{t,p} = \begin{bmatrix}
%         r_{t-p+1}^T & r_{t-p+2}^T & \dots & r_t^T 
%         % r_{t-p+2} \\
%         % \vdots \\
%         % r_{t}
%     \end{bmatrix}^T
% \end{equation}
% and $p$ denotes the memory of the system. We assume that the dynamics \ref{eq:dynamics} are stable, meaning that $M_t \in \mathcal{M} \triangleq \{M\in\mathbb{R}^{n\times pn} \ | \ \norm{M} \leq D\}$, for some $D\geq 0$, for all $t\geq 0$. 



% \subsection{Target Dynamics}
% We consider the case where the data we wish to predict is generated by a \textit{partially observable system}, meaning that the state $r_t$ at time $t$ depends on the past $p$ states, as
% \begin{equation}
%     r_{t+1} = M_t r_{t,p}
% \end{equation}
% where
% \begin{equation}
%     r_{t,p} = \begin{bmatrix}
%         r_{t-p+1}^T & r_{t-p+2}^T & \dots & r_t^T 
%         % r_{t-p+2} \\
%         % \vdots \\
%         % r_{t}
%     \end{bmatrix}^T
% \end{equation}

% \tasos{these should go to subsection a}
% Our proposed Residuals Offline-Online Method, schematically shown in Fig. \ref{fig:res-off-on}, aims to learn online the residuals errors of the offline experts. Assuming $N$ offline experts, their residual errors are defined as:
% \begin{equation}
%     e_{t,i} = \hat{r}_{t,i}^{\text{off}} - r_t
% \end{equation}
% where $r_t$ is the ground truth and $i\in\{1,2,\dots,N\}$ is the Expert index. \tasos{I don't understand this, why take fully observed here? is this a choice for pedestrian tracking?} We make the assumption that these residual errors act as a \textit{fully observable system} ($p=1$) and we attempt to learn them online. Finally, we combine them online using the Meta Algorithm \ref{alg:meta_alg}. If successful, this method indicates that the residual errors evolve as an affine system:
% \begin{equation}
%     e_{t+1,i} = M_{t,i}e_{t,i} + w_{t,i}\tasos{\text{notation clash}}
%     \label{eq:error_dynamics}
% \end{equation}
% which can be written in the form of \ref{eq:dynamics} if we consider the augmented state $\bar{e}_{t,i} = \begin{bmatrix}
%     e_{t,i}^T & 1
% \end{bmatrix}^T$.

% \tasos{first present the online adaptation within every expert and then across experts. So this should be combined with subsection a}



% In order to predict the residual errors online, we will use the \emph{Recursive Least Squares} (RLS) Algorithm \cite{yuan2020trading}. This algorithm aims to minimize the following cost:
% \begin{equation}
%     J_t(M_i) = \sum_{\tau=p+k-1}^t \gamma_i^{t-\tau} \norm{e_{\tau,i} - M_i e_{\tau-k-p+1:\tau-k,i}}
%     \label{eq:cost}
% \end{equation}
% % where $\ell_t(M_i) = \norm{e_{t,i} - M_ie_{t-k,i}}^2 $ 
% for each expert $i\in\{1,2,\dots,N\}$ and it enjoys recursive update based on the current data. Notice that we have introduced forgetting factors $\gamma_i$ in order to be able to adapt to changing dynamics. 

For the case of $k$-steps ahead prediction, we initialize $k$ independent learners $\hat{M}_{j+k|j, i}, \ j\in\{0,1,\dots,k-1\}$ and we minimize the cost \eqref{eq:cost} recursively as described in~\cref{alg:RLS} for each $i\in\{1,2,\dots,N\}$. 
 

% $\hat{M}_{1,i}^{(0)}, \dots \hat{M}_{1,i}^{(k)}$ for each expert $i$ and we perform the following recursive update \cite{}:
% \begin{align}
% \begin{split}
% P_{t|t-k,i}^{(j)} &= \gamma P_{t-k|t-2k, i}^{(j)} + e_{t-k,i} e_{t-k,i}^T \\
% \hat{M}_{t+k|t, i}^{(j)} &= \hat{M}_{t|t-k, i}^{(j)} + (e_{t,i} - \hat{M}_{t|t-k, i}^{(j)} e_{t-k,i})e_{t-k,i}^T (P_{t|t-k, i}^{(j)}) ^{-1} \\
% \hat{e}_{t+k|t, i} &= \hat{M}_{t+k|t, i}^{(j)} e_{t,i}
% \end{split}
% \end{align}
% where $j$ denotes the learned index. 

\begin{algorithm}
    \caption{k-steps ahead RLS prediction}
    \label{alg:RLS}
    \begin{algorithmic}
        \Require Forgetting factor $\gamma_i \in (0,1)$ for expert $i\in\{1,2,\dots,N\}$
        \State Initialize $k$ learners $\hat{M}_{j+k, i}, \ j\in\{0,1,\dots,k-1\}$ 
        \State Initialize $P_{j, i} = \mathbb{I}$, $j \in\{0,1,\dots,k-1\}$
        \For{$t=k,\dots,T$} 
        \State Make prediction $\hat{e}_{t,i} = \hat{M}_{t,i}z_{t-k,i}$
        \State Receive true state $r_t$, compute residual error $e_{t,i}$ 
        \State Incur loss $\ell_t(\hat{M}_{t,i}) = \norm{e_{t,i} - \hat{e}_{t,i}}^2$
        % \State Learner index: $j = t \mod k$
        % \State $i = \lceil \frac{t}{k} \rceil$
        \State Update $P_{t,i} = \gamma_i P_{t-k, i} + z_{t-k,i} z_{t-k,i}^{\top}$
        % \begin{align*}            
        %     P_{t,i} = \gamma_i P_{t-k, i} + z_{t-k,i} z_{t-k,i}^{\top}
        % \end{align*}
        % % $P_{t,j} = \gamma P_{t,j} + r_{t-k,p}r_{t-k,p}^T $
        \State Update $\hat{M}_{t+k, i} = \hat{M}_{t, i} + (e_{t,i} - \hat{M}_{t, i} z_{t-k, i})z_{t-k, i}^{\top} P_{t, i} ^{-1}$
        % \begin{align*}
        % \hat{M}_{t+k, i} = \hat{M}_{t, i} + (e_{t,i} - \hat{M}_{t, i} z_{t-k, i})z_{t-k, i}^{\top} P_{t, i} ^{-1}
        % \end{align*}
        % % \[\hat{M}_{t+1,j} = \hat{M}_{t,j} + \left(r_t - \hat{M}_{t,j} r_{t-k,p} \right) r_{t-k,p}^T (P_{t,j})^{-1}\]
        % \State Make prediction $r_{t+k|t} = \hat{M}_{t+1|k,j} r_{t,p}$
        
        % \If{$t - p \geq k$}
        % \State Incur cost $\ell_t(\hat{M}_{t|t-k,j}) =  \norm{r_t - \hat{M}_{t|t-k,j} r_{t-k,p}}^2$
        % \State Update $P_{t|t-k,j} = \gamma P_{t-k|t-2k, j} + r_{t-k,p} r_{t-k,p}^T$
        % % $P_{t,j} = \gamma P_{t,j} + r_{t-k,p}r_{t-k,p}^T $
        % \State Update \[\hat{M}_{t+k|t, j} = \hat{M}_{t|t-k, j} + (r_t - \hat{M}_{t|t-k, j} r_{t-k, p})r_{t-k, p}^T P_{t|t-k, j} ^{-1}\]
        % % \[\hat{M}_{t+1,j} = \hat{M}_{t,j} + \left(r_t - \hat{M}_{t,j} r_{t-k,p} \right) r_{t-k,p}^T (P_{t,j})^{-1}\]
        % \State Make prediction $r_{t+k|t} = \hat{M}_{t+1|k,j} r_{t,p}$
        % \Else
        % \State Make prediction $r_{t+k|t} = r_t$
        % \EndIf
        \EndFor
        
    \end{algorithmic}
\end{algorithm}

\subsection{Combining Multiple Predictions}
In order to combine online the multiple residuals predictions, we introduce the general notion of Prediction with Experts Advice \cite{cesa2006prediction}. More specifically, we 
% \tasos{we already assumed that we have those. Maybe say we treat the offline predictions+RLS as experts}
treat the $N$ residual errors predictions as Experts, and we assign weights (levels of trust) to each of them. These weights are adaptively updated using softmax on the errors of each expert. Finally, the aggregate prediction is the sum of the weighted experts predictions. The whole procedure is summarized in \cref{alg:meta_alg}, which is called \emph{Meta Algorithm}. For simplicity reasons, we have adopted the abbreviated notation of $\hat{e}_{t,i} = \hat{e}_{t|t-k,i}$.

%We propose two methods, the so-called \textit{Expert Offline-Online} and \textit{Residuals Offline-Online}, with the second one building on top of the first. 

% \subsubsection{Expert Offline-Online}

% \begin{figure}
%     \centering
%     \includegraphics[scale=0.12]{expert-offline-online.eps}
%     \caption{Schematic of Expert Offline-Online method. The Offline Model produces $N$ Offline Predictions-Experts, which are combined online. We can also append a purely online Expert, in order to boost performance.}
%     \label{fig:expert-offline-online}
% \end{figure}

\begin{algorithm}
    \caption{Meta-Algorithm for Prediction with Experts Advice}
    \label{alg:meta_alg}
    % \footnotesize
    \begin{algorithmic}
        \Require Learning rate $\lambda$, set of $N$ experts $\mathcal{E}_N = \{E_i|i=1,\dots,N\}$
        \State Assign weights $w_{1,1}= w_{1,2}=\dots= w_{0,N}=\frac{1}{N}$ to each Expert.
        \For{$t=1,2,\dots,T$} 
        \State Obtain prediction $\hat{e}_{t,i}$ from each Expert $i$.
        \State $\hat{r}_{t,i} = \hat{r}_{t,i}^{\mathrm{off}} + \hat{e}_{t,i}$ for each Expert $i$.
        \State Aggregate prediction $\hat{r}_t = \sum_i w_{t,i} \hat{r}_{t,i}$
        \State Compute losses $\ell_{t}(\hat{r}_{t,1}), \dots, \ell_{t}(\hat{r}_{t,N})$ for each Expert
        \State Update the weights as 
        \begin{equation*}
            w_{t+1,i} = \frac{w_{t,i} \exp(-\lambda \ell_{t}(\hat{r}_{t,i}))}{\sum_i w_{t,i} \exp(-\lambda \ell_{t}(\hat{r}_{t,i}))}
        \end{equation*}
        \EndFor
    \end{algorithmic}
\end{algorithm}
% We also explore including a purely online Expert, in order to steer the aggregate prediction towards the ground truth.



% \subsubsection{Residuals Offline-Online} 
% The Residuals Offline-Online method, schematically shown in Fig. \ref{fig:res-off-on}, assumes again $N$ Offline Experts, and we define their residual errors as:
% \begin{equation}
%     e_{t,i}^{\text{res}} = \hat{r}_{t,i}^{\text{off}} - r_t
% \end{equation}
% where $r_t$ is the ground truth and $i\in\{1,2,\dots,N\}$. We make the assumption that these residual errors act as a \textit{fully observable system} ($p=1$) and we attempt to learn them online using the RLS Algorithm \ref{alg:RLS}. In case of multiple residual errors, we again combine them online using the Meta Algorithm \ref{alg:meta_alg}. If successful, this method indicates that the residual errors evolve as an affine system:
% \begin{equation}
%     e_{t+1,i} = A_{t,i}e_{t,i} + w_{t,i}
% \end{equation}

% \subsection{Online Prediction}

% Notice that for timesteps $t < k + p$ we use a \textit{Naive Predictor} $r_{t+k|t} = r_t$. This addition does not affect the overall prediction performance.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

